MPQ-DM: Mixed Precision Quantization for Extremely Low Bit Diffusion Models

Diffusion models have received wide attention in generation tasks. However, the expensive computation cost prevents the application of diffusion models in resource-constrained scenarios. Quantization emerges as a practical solution that significantly saves storage and computation by reducing the bit-width of parameters. However, the existing quantization methods for diffusion models still cause severe degradation in performance, especially under extremely low bit-widths (2-4 bit). The primary decrease in performance comes from the significant discretization of activation values at low bit quantization. Too few activation candidates are unfriendly for outlier significant weight channel quantization, and the discretized features prevent stable learning over different time steps of the diffusion model. This paper presents MPQ-DM, a Mixed-Precision Quantization method for Diffusion Models. The proposed MPQ-DM mainly relies on two techniques:(1) To mitigate the quantization error caused by outlier severe weight channels, we propose an Outlier-Driven Mixed Quantization (OMQ) technique that uses $Kurtosis$ to quantify outlier salient channels and apply optimized intra-layer mixed-precision bit-width allocation to recover accuracy performance within target efficiency.(2) To robustly learn representations crossing time steps, we construct a Time-Smoothed Relation Distillation (TRD) scheme between the quantized diffusion model and its full-precision counterpart, transferring discrete and continuous latent to a unified relation space to reduce the representation inconsistency. Comprehensive experiments demonstrate that MPQ-DM achieves significant accuracy gains under extremely low bit-widths compared with SOTA quantization methods. MPQ-DM achieves a 58\% FID decrease under W2A4 setting compared with baseline, while all other methods even collapse.

==> sec/3_preliminary.tex <==
\section{Preliminary}
\subsection{Model Quantization}
Model quantization maps model weights and activations to low bit integer values to reduce memory footprint and accelerate the inference. For a floating vector $\mathbf{x}_f$, the quantization process can be formulated as:
\begin{equation}
\begin{gathered}
    \hat{\mathbf{x}}_q = Q(\mathbf{x}_f, s, z) = clip(\lfloor \frac{\mathbf{x}_f}{s} \rceil + z, 0, 2^N-1) \\
    s = \frac{u-l}{2^N-1}, z = - \lfloor \frac{l}{s} \rceil
\end{gathered}
\end{equation}
where $\hat{\mathbf{x}}_q$ indicates quantized vector in integer, $\lfloor \cdot \rceil$ is round fuction and $clip(\cdot)$ is function that clamps values into the range of $[0, 2^N-1]$, $s$ is a scale factor and $z$ is a quantization zero point. $l$ and $u$ are the lower and upper bounds of quantization thresholds respectively. They are determined by $\mathbf{x}_f$ and the target bit-width.
Reversely, in order to restore the low precision integer quantization vector $\hat{\mathbf{x}}_q$ to the full precision representation, the dequantization process is formulated as:
\begin{equation}
    \hat{\mathbf{x}}_f = \hat{Q}(\mathbf{x}_f) = (\hat{\mathbf{x}}_q - z)  s
\end{equation}
where $\hat{\mathbf{x}}_f$ is the dequantized vector used for forward process.

\iffalse
\subsection{Quantization-aware Efficient Fine-tuning}
Post-training quantization (PTQ) and Quantization-aware
training (QAT) are two main approaches for model quantization. Although the PTQ methods greatly reduces the training cost without fine-tuning the model weights, it often shows a huge performance degradation at low bit. However, the traditional QAT methods can guarantee the quantization performance at low Bit, but it requires a large amount of training time to ensure convergence due to the training of original model weights. In order to reduce the memory and time consumption in the QAT training of the diffusion model, EfficientDM proposes to fine-tuning the additional module QA-LoRA instead of fine-tuning all model weights. Low-rank adapter (LoRA) fine-tuning constrains the update of the model parameters to possess a low intrinsic rank, denoted as r. Given a pretrained linear module weight $\mathbf{W} \in \mathbb{R}^{c_{in}\times c_{out}}$, $c_{in}$ and $c_{out}$ representing the number of input and output channels, respectively. LoRA fixes the original weights $\mathbf{W}$ and introduces updates as follows:
\begin{equation}
    \mathbf{W} = \mathbf{W} + \mathbf{B}\mathbf{A}
\end{equation}
where $\mathbf{B} \in \mathbb{R}^{c_{in}\times r}$ and $\mathbf{A} \in \mathbb{R}^{r\times c_{out}}$ are the learnable two low-rank matrices with $r \ll min(c_{in}, c_{out})$, thus the number of parameters for fine-tuning $\mathbf{B}\mathbf{A}$ is much lower than fine-tuning the original weight $\mathbf{X}$. With QA-LoRA module, the quantization process of model weight in fine-tuning stage can be formulated as:
\begin{equation}
    \hat{\mathbf{W}}_q = Q(\mathbf{W}_f + \mathbf{B}\mathbf{A}, s, z)
\end{equation}
where $\mathbf{W}_f$ is the original floating-point weight of the model that does not need to be updated, and $\mathbf{B}\mathbf{A}$ is the low-rank weight of QA-LoRA module that will be updated. After the fine-tuning stage, the QA-LoRA weight will be added to the original weight to form a new weight matrix and sharing the same scale fator and quantization zero point without additional memory footprint.
\fi


==> sec/checklist.tex <==
\paragraph{This paper:}
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA) {\bf yes}
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no) {\bf yes}
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no) {\bf yes}
\end{itemize}

\paragraph{Does this paper make theoretical contributions? (yes/no)}
{\bf no}

If yes, please complete the list below.

\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
    \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
    \item Proofs of all novel claims are included. (yes/partial/no)
    \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
    \item Appropriate citations to theoretical tools used are given. (yes/partial/no)
    \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
    \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
\end{itemize}

\paragraph{Does this paper rely on one or more datasets? (yes/no)}
{\bf yes}

If yes, please complete the list below.

\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA) {\bf yes}
    \item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA) {\bf NA}
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA) {\bf NA}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA) {\bf yes}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA)
    {\bf yes}
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA) {\bf NA}
\end{itemize}

\paragraph{Does this paper include computational experiments? (yes/no)}
{\bf yes}

If yes, please complete the list below.

\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. (yes/partial/no). {\bf yes}
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no) {\bf partial}
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no) {\bf yes}
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no) {\bf yes}
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA) {\bf NA}
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no) {\bf yes}
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no) {\bf yes}
    \item This paper states the number of algorithm runs used to compute each reported result. (yes/no) {\bf yes}
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no) {\bf no}
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no) {\bf yes}
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA) {\bf yes}
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA) {\bf yes}
\end{itemize}

